Mutual Inclusivity of the Critical Path and its Partial Schedule on Heterogeneous Systems

The critical path of a group of tasks is an important measure that is commonly used to guide task allocation and scheduling on parallel computers. The critical path is the longest chain of dependencies in an acyclic task dependence graph. A problem arises on heterogeneous parallel machines where computation and communication costs can vary between different types of processor. Existing solutions for heterogeneous machines attempt to estimate the critical path using average values of computation and communication costs. However, this ignores opportunities to match specific tasks to specific classes of processor and communication links, and can result in quite misleading paths being identified as critical. We argue that an accurate critical path must consider the mapping of tasks to classes of processor and communication links. We formulate a polynomial time algorithm to find such a critical path. Our Critical Earliest Finish Time (CEFT) algorithm finds both the length of the critical path and an allocation of tasks to processors on that path. We compared CEFT experimentally to existing approaches such as averaging execution times across processors. The latter approach fails to accurately model the execution cost of tasks, and as a result fails to identify a correct critical path in 83.99% of cases in our experiments. We also adapted a critical path-oriented scheduling algorithm (CPOP) to use our critical path algorithm and found that the resulting schedules are faster.

==> Makefile <==
dirName = `basename $(PWD)`
currentDate = `date +%D | sed 's/\//-/g'`
fileName = ../$(dirName)-$(currentDate).tar.gz
all: *.tex Makefile *.cls
	pdflatex main
	-bibtex main
	pdflatex main
	pdflatex main

.PHONY: clean backup
clean:
	rm -f *.log *.dvi *.toc *.aux *.bbl *.blg

backup:
	tar --exclude=*git* --exclude=*input* --exclude=*output* --exclude=.git* -czvf $(fileName) $(PWD)/*


==> aravind.tex <==

%\section{Aravind's ramblings}
%\label{sec:arav-ramb}
%
%%Perhaps we should stop calling this new method the Dynamic Programming approach. From the looks of it, we have to break pattern for the last/exit nodes anyway in order to calculate the makespan of the critical path (\aravind{maybe we don't have to, must investigate further}). Our method being a Dynamic Programming approach is its defining characteristic but its not unique characteristic. All of our competitors (HEFT, PEFT, SDC) etc are all DP based approaches as well.
%
%Pitfalls with contemporary methods of identifying Critical Path in a heterogeneous computing environment:
%\aravind
%{
%\begin{itemize}
%	\item Obfuscates heterogeneity in resources by averaging execution times.
%	\item Obfuscates heterogeneity in bandwidth by averaging transfer latencies.
%	\item True critical path is never found.
%	\item 
%\end{itemize}
%}
%
%Your method seems interesting, but why do we need to find out the ``Critical Path'' of a graph at all? Importance of the  Critical Path:
%\aravind
%{
%\begin{itemize}
%\item 
%\end{itemize}
%}

%To extend this algorithm to schedule a whole DAG to minimize its makespan, we need to do the following:
%\aravind
%{
%\begin{itemize}
%	\item Have a task prioritization phase or have a way to walk the graph (most likely BFS)
%	\item In the processor selection phase we either:
%	\begin{itemize}
%		\item Run our MapPath (Algorithm~\ref{algo:map-path}) on every path from source to sink. This will be very costly.
%		\item Run MapPath's logic on tasks by accounting for all their parents instead of just one parent (previousTask). This will make the algorithm $O(\averageDegree\numberOfTasks\numberOfResources^2)$ where $\averageDegree$ is the average in-degree of the application graph.
%	\end{itemize}
%	\item Include some sense of processor availability. Current versions of our algorithm assumes processors are instantly available.
%\end{itemize}
%}

%\begin{algorithm}
%	\caption{Calculating Ranks As A Measure Of Distance From Critical Path}
%	\label{algo:calcdistanceranks}
%	\begin{algorithmic}[1]
%	\Require Algorithm ~\ref{algo:calcinitsolnSA} must've been run and a valid $CP$ is at hand
%	\Statex
%	\Function{CalcRanks}{$G_t, \Omega(CP)$}
%		\Let{$Rank_{Down}(\mathcal{T})$}{The downward rank of each $t_i \in \mathcal{T}$} \Comment{$\mathcal{T}$ is the task set}
%		\For {$i=0 \cdots n_\mathcal{T}-1$} \Comment{$n_\mathcal{T}=|V_\mathcal{T}|$}
%			\If {$t_i \in CP$} \Comment{If task is in CP}
%				\State $Rank_{Down}(t_i) \gets 0 $ 
%			\Else
%				\Let{$Rank_{Down}(t_i)$}{$\underset{\forall t_j \in pred(t_i)}{min}(Rank_{Down}(t_j)) + 1$}
%			\EndIf
%		\EndFor
%		\Let{$Rank_{Up}(\mathcal{T})$}{The upward rank of each $t_i \in \mathcal{T}$}
%		\For {$i=n_\mathcal{T}-1 \cdots 0$}
%			\If {$t_i \in CP$}
%				\State $Rank_{Up}(t_i) \gets 0 $ 
%			\Else
%				\Let{$Rank_{Up}(t_i)$}{$\underset{\forall t_j \in succ(t_i)}{min}(Rank_{Up}(t_j)) + 1$}
%			\EndIf
%		\EndFor
%		\Let{$\underset{\Omega(CP)}{Rank}(\mathcal{T})$}{$Rank_{Down}(\mathcal{T}) + Rank_{Up}(\mathcal{T})$}; $\forall t_i \in \mathcal{T}$
%	\State \Return{$\underset{\Omega(CP)}{Rank}(\mathcal{T})$}
%	\EndFunction
%	\end{algorithmic}
%\end{algorithm}
